Hierarchical Bayesian CMB Component Separation with the No-U-Turn Sampler

In this paper we present a novel implementation of Bayesian CMB component separation. We sample from the full posterior distribution using the No-U-Turn Sampler (NUTS), a gradient-based sampling algorithm. Alongside this, we introduce new foreground modelling approaches. We use the mean-shift algorithm to define regions on the sky, clustering according to naively estimated foreground spectral parameters. Over these regions we adopt a complete pooling model, where we assume constant spectral parameters, and a hierarchical model, where we model individual pixel spectral parameters as being drawn from underlying hyper-distributions. We validate the algorithm against simulations of the \textit{LiteBIRD} and C-BASS experiments, with an input tensor-to-scalar ratio of $r=5\times 10^{-3}$. Considering multipoles $30\leq\ell<180$, we are able to recover estimates for $r$. With \textit{LiteBIRD}-only observations, and using the complete pooling model, we recover $r=(12.9\pm 1.4)\times 10^{-3}$. For C-BASS and \textit{LiteBIRD} observations we find $r=(9.0\pm 1.1)\times 10^{-3}$ using the complete pooling model, and $r=(5.2\pm 1.0)\times 10^{-3}$ using the hierarchical model. Unlike the complete pooling model, the hierarchical model captures pixel-scale spatial variations in the foreground spectral parameters, and therefore produces cosmological parameter estimates with reduced bias, without inflating the their uncertainties. Measured by the rate of effective sample generation, NUTS offers performance improvements of $\sim10^3$ over using Metropolis-Hastings to fit the complete pooling model. The efficiency of NUTS allows us to fit the more sophisticated hierarchical foreground model, that would likely be intractable with non-gradient based sampling algorithms.

==> nuts_algo.tex <==
\section{The No-U-Turn Sampler}\label{sec: nuts algo}

At its core, the NUTS algorithm is an extension of HMC, which was originally developed for performing calculations in lattice field theory \citep{DUANE1987216}. In this section we give an overview of the HMC algorithm, and the additional tuning procedures NUTS implements to avoid the need for hand-tuned HMC implementations. For a detailed discussion of NUTS and HMC see \cite{Homan:2014:NSA:2627435.2638586,doi:10.1111/2041-210X.12681,2017arXiv170102434B,betancourt2017}.

HMC essentially proceeds by simulating Hamiltonian trajectories through parameter space. A simple implementation may proceed as follows:
\begin{enumerate}
	\item Given a set of parameters, $\mathbf{\Theta}=\left[\Theta_{1},\ldots,\Theta_{D}\right]$, with corresponding joint density, $p\left(\mathbf{\Theta}\right)$, we introduce a corresponding set of auxiliary momentum variables $\mathbfit{r}=\left[r_{1},\ldots,r_{D}\right]$. We take the distribution over the momenta to be a Gaussian distribution centered on zero, i.e., $\mathbfit{r}\sim\mathcal{N}(\mathbf{0},\mathbfss{M})$, where $\mathbfss{M}$ is the mass matrix. This defines a kinetic energy term,
	\begin{equation}
	    K(\mathbf{\Theta},\mathbfit{r}) =  \frac{1}{2}\mathbfit{r}^{\top}\mathbfss{M}^{-1}\mathbfit{r} + \ln{\left|\mathbfss{M}\right|} + \mathrm{const.}
	\end{equation}
	We may then define the Hamiltonian of our system as,
	\begin{equation}
	    \mathcal{H}(\mathbfit{r},\mathbf{\Theta}) = -\ln p(\mathbfit{r}|\mathbf{\Theta}) - \ln p\left(\mathbf{\Theta}\right). = K(\mathbf{\Theta},\mathbfit{r}) + V\left(\mathbf{\Theta}\right),
	\end{equation}
	where we define the potential energy term, $V\left(\mathbf{\Theta}\right) = - \ln p\left(\mathbf{\Theta}\right)$.
    \item We then evolve our position in parameter space by integrating Hamilton's equations,
    \begin{align}
        \frac{\mathrm{d}\mathbf{\Theta}}{\mathrm{d}t} &= \frac{\partial\mathcal{H}}{\partial\mathbfit{r}},\\
        \frac{\mathrm{d}\mathbfit{r}}{\mathrm{d}t} &= -\frac{\partial\mathcal{H}}{\partial\mathbf{\Theta}}.
    \end{align}
    Practically this is done through a leapfrog algorithm. To generate a new sample in our Markov chain we draw $\mathbfit{r}$ from $\mathcal{N}(\mathbf{0}, \mathbfss{M})$. The leapfrog steps then proceed as,
    \begin{align}
	&\mathbfit{r}^{t+\epsilon/2} = \mathbfit{r}^{t} - \frac{\epsilon}{2}\nabla_{\mathbf{\Theta}}V(\mathbf{\Theta}^{t}),\\
	&\mathbf{\Theta}^{t+\epsilon} = \mathbf{\Theta}^{t} + \epsilon\mathbfss{M}\mathbfit{r}^{t+\epsilon/2},\\
	&\mathbfit{r}^{t+\epsilon} = \mathbfit{r}^{t+\epsilon/2}-\frac{\epsilon}{2}\nabla_{\mathbf{\Theta}}V(\mathbf{\Theta}^{t+\epsilon}),
	\end{align}
	where $\epsilon$ is the leapfrog step-size. The leapfrog steps used to update our position have the convenient property of being a symplectic integrator. That is, the numerical trajectory generated by the leapfrog steps preserve the volume of phase space, as is the case for the Hamiltonian trajectories they approximate. A more detailed discussion of the numerical integration of Hamilton's equations can be found in \ref{2005shd..book.....L}. These leapfrog steps are performed $L$ times to generate a new proposal position, $\left(\mathbf{r}^*,\mathbf{\Theta}^*\right)$.
	\item The new proposal position is then accepted with a probability of acceptance being given by,
	\begin{equation}
	    p_{\alpha} = \mathrm{min}\left\{1, \exp\left(\mathcal{H}(\mathbfit{r},\mathbf{\Theta}) - \mathcal{H}(\mathbfit{r}^*,\mathbf{\Theta}^*)\right)\right\}.
	\end{equation}
	We may note that what we have done here is essentially generate a Metropolis-Hastings proposal step with a very high chance of being accepted.
	\item By repeating this sampling procedure $N$ times over we may generate the parameter samples for our Markov chain.
\end{enumerate}

The mass matrix used to define the distribution over the momenta acts to rotate and re-scale parameter space. Choosing $\mathbfss{M}^{-1}$ to be the covariance of the target distribution will help to de-correlate the target distribution, which can lead to significant performance improvements when dealing with highly correlated parameters. For practical implementations the mass matrix can be estimated during a tuning phase. Starting with the identity matrix we can generate an initial sample set, from which we update our estimate of the mass matrix using the sample covariance. We may then iterate over this tuning process to generate an accurate estimate of the covariance of the target distribution \citep{2017arXiv170102434B}. Whilst estimating off-diagonal elements of the mass matrix does help in de-correlating the target distribution, using the off-diagonal elements does not necessarily scale well to high dimensional problems given the need to invert the mass matrix at the end of tuning, and perform matrix multiplications during leapfrog steps. For our analysis in this paper, tuning the full mass matrix does not offer any performance improvements. However, this can significantly improve sampling efficiency for single pixel analyses, or analyses assuming complete independence between pixels. In this case, one can employ the tuning steps in \cite{exoplanet:exoplanet}, using the default tuning schedule described in \cite{stan_development_team_stan_2012}.

The efficiency of HMC as described above critically depends on the choice of $\epsilon$ and $L$ used in the leapfrog steps. If $\epsilon$ is chosen to be too small, the sampler will waste computation taking very small steps along the Hamiltonian trajectories. In contrast, if $\epsilon$ is chosen to be too large, the simulation of the Hamiltonian trajectory will become inaccurate and the sampler will produce proposal steps with low acceptance probabilities. If $L$ is chosen to be too small, the sampler will generate samples close to one another, resulting in undesirable random walk behaviour. If $L$ is chosen to be too large on the other hand, the sampler will generate paths through parameter space that loop back on themselves. This results in proposal steps close to the starting value, with the additional waste of generating the extended trajectory. In even more severe scenarios, a poor choice of $L$ that results in the sampler jumping from one side of parameter space to another at each iteration can result in a non-ergodic chain i.e. a chain that is not guaranteed to converge on the target distribution \citep{neal_mcmc_hmc2012}. 

The need to finely tune $\epsilon$ and $L$ means that standard implementations of HMC typically require costly tuning runs. This can significantly reduce the utility and general applicability of HMC in realistic problems. The NUTS algorithm overcomes these problems by automatically tuning these sampling parameters. The value of $\epsilon$ is tuned during an initial tuning phase to meet some target acceptance probability. The target acceptance probability can be adjusted depending on the degree of curvature in the posterior, with a higher acceptance rate (or equivalently, smaller step-size) being needed for more problematic distributions. The value of $L$ is modified during sampling to meet a No-U-Turn criterion. That is, the leapfrog integrator is iterated over until the simulated trajectory begins to turn back on itself, or a maximum depth is reached for the simulation. In doing so, the sampler is able to maximize the distance between the proposal step and the initial position, before looping back on itself and wasting computation. For details on this tuning we refer the reader to \ref{Homan:2014:NSA:2627435.2638586,stan_development_team_stan_2012,pymc3_citation}.


